Multi-Cycle Assignment Problems with Rotational Diversity

Multi-cycle assignment problems address scenarios where a series of general assignment problems has to be solved sequentially. Subsequent cycles can differ from previous ones due to changing availability or creation of tasks and agents, which makes an upfront static schedule infeasible and introduces uncertainty in the task-agent assignment process. We consider the setting where, besides profit maximization, it is also desired to maintain diverse assignments for tasks and agents, such that all tasks have been assigned to all agents over subsequent cycles. This problem of multi-cycle assignment with rotational diversity is approached in two sub-problems: The outer problem which augments the original profit maximization objective with additional information about the state of rotational diversity while the inner problem solves the adjusted general assignment problem in a single execution of the model. We discuss strategies to augment the profit values and evaluate them experimentally. The method's efficacy is shown in three case studies: multi-cycle variants of the multiple knapsack and the multiple subset sum problems, and a real-world case study on the test case selection and assignment problem from the software engineering domain.

==> figures/avail_size_mcmssp_60.tex <==

\begin{tabular}{lllllll}
\toprule
                  & Avail. Agents & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{5} &          All \\
                  & Avail. Tasks & \multicolumn{2}{l}{20} & \multicolumn{3}{l}{20} \\
                  & agentavail & \multicolumn{2}{l}{100} & \multicolumn{3}{l}{100} \\
                  & taskavail &           50 &           75 &         50 & \multicolumn{2}{l}{75} \\
{} &  &              &              &            &            &              \\
\midrule
Rotational Diversity & FOA &  29.0 (45.4) &  28.0 (55.5) &  4.0 (7.8) &  5.0 (9.5) &  16.0 (29.6) \\
                  & PC &  30.0 (44.1) &  41.0 (49.8) &  5.0 (7.6) &  5.0 (9.0) &  20.0 (27.6) \\
                  & FOP &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  0.0 (6.6) &  13.0 (25.6) \\
                  & OS/1 &  32.0 (44.9) &  29.0 (55.5) &  5.0 (7.6) &  6.0 (9.5) &  18.0 (29.4) \\
                  & OS/1 &  32.0 (44.9) &  29.0 (55.5) &  4.0 (7.5) &  5.0 (9.4) &  17.0 (29.3) \\
                  & OS/10 &  27.0 (43.7) &  28.0 (47.8) &  1.0 (4.6) &  2.0 (7.6) &  14.0 (25.9) \\
                  & OS/10 &  27.0 (43.7) &  28.0 (47.8) &  2.0 (6.7) &  3.0 (8.8) &  15.0 (26.8) \\
                  & switch15 &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  2.0 (7.1) &  14.0 (25.8) \\
                  & switch15-limit &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  2.0 (8.5) &  14.0 (26.7) \\
                  & OS/2 &  28.0 (44.0) &  36.0 (51.9) &  4.0 (7.0) &  5.0 (9.4) &  18.0 (28.1) \\
                  & OS/2 &  28.0 (44.0) &  36.0 (51.9) &  4.0 (7.2) &  5.0 (9.5) &  18.0 (28.2) \\
                  & OS/20 &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  1.0 (7.0) &  14.0 (25.7) \\
                  & OS/20 &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  1.0 (8.6) &  14.0 (26.7) \\
                  & switch25 &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  1.0 (6.9) &  14.0 (25.7) \\
                  & switch25-limit &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  1.0 (8.6) &  14.0 (26.7) \\
                  & OS/3 &  27.0 (43.7) &  35.0 (50.0) &  4.0 (6.4) &  5.0 (9.4) &  17.0 (27.4) \\
                  & OS/3 &  27.0 (43.7) &  35.0 (50.0) &  4.0 (7.1) &  5.0 (9.4) &  17.0 (27.6) \\
                  & OS/30 &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  1.0 (6.9) &  14.0 (25.7) \\
                  & OS/30 &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  1.0 (8.6) &  14.0 (26.7) \\
                  & switch35 &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  0.0 (6.8) &  13.0 (25.7) \\
                  & switch35-limit &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  0.0 (8.6) &  14.0 (26.7) \\
                  & OS/4 &  27.0 (43.7) &  31.0 (49.0) &  3.0 (5.7) &  5.0 (9.1) &  16.0 (26.9) \\
                  & OS/4 &  27.0 (43.7) &  31.0 (49.0) &  4.0 (7.0) &  5.0 (9.3) &  16.0 (27.2) \\
                  & OS/40 &  27.0 (43.7) &  27.0 (47.8) &  1.0 (4.4) &  0.0 (6.7) &  13.0 (25.7) \\
                  & OS/40 &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  0.0 (8.7) &  14.0 (26.7) \\
                  & switch5 &  27.0 (43.7) &  31.0 (48.4) &  3.0 (5.6) &  4.0 (8.7) &  16.0 (26.6) \\
                  & switch5-limit &  27.0 (43.7) &  31.0 (48.4) &  4.0 (7.0) &  4.0 (8.8) &  16.0 (27.0) \\
                  & switch6 &  27.0 (43.7) &  29.0 (48.4) &  2.0 (5.1) &  4.0 (8.2) &  15.0 (26.4) \\
                  & switch6-limit &  27.0 (43.7) &  29.0 (48.4) &  3.0 (6.9) &  4.0 (8.9) &  15.0 (27.0) \\
                  & switch7 &  27.0 (43.7) &  29.0 (48.2) &  2.0 (5.1) &  4.0 (7.9) &  15.0 (26.2) \\
                  & switch7-limit &  27.0 (43.7) &  29.0 (48.2) &  3.0 (6.8) &  3.0 (8.7) &  15.0 (26.8) \\
                  & switch8 &  27.0 (43.7) &  28.0 (48.0) &  2.0 (4.8) &  3.0 (8.0) &  15.0 (26.1) \\
                  & switch8-limit &  27.0 (43.7) &  28.0 (48.0) &  3.0 (6.9) &  3.0 (8.8) &  15.0 (26.8) \\
                  & switch9 &  27.0 (43.7) &  28.0 (48.0) &  2.0 (4.8) &  3.0 (7.8) &  15.0 (26.1) \\
                  & switch9-limit &  27.0 (43.7) &  28.0 (48.0) &  3.0 (6.9) &  3.0 (8.8) &  15.0 (26.8) \\
                  & WPP &  30.0 (43.7) &  38.0 (48.4) &  5.0 (7.4) &  6.0 (9.0) &  19.0 (27.2) \\
                  & All &  27.0 (43.9) &  29.0 (49.0) &  2.0 (6.1) &  2.0 (8.4) &  15.0 (26.9) \\
Profit (\% of FOP) & FOA &         96.4 &           95 &       95.5 &       92.9 &         94.9 \\
                  & PC &         99.9 &         99.9 &       97.6 &         95 &         98.1 \\
                  & FOP &          100 &          100 &        100 &        100 &          100 \\
                  & OS/1 &         97.8 &         95.2 &         96 &         93 &         95.5 \\
                  & OS/1 &         97.8 &         95.2 &       95.3 &       92.7 &         95.2 \\
                  & OS/10 &          100 &          100 &       99.8 &       97.7 &         99.4 \\
                  & OS/10 &          100 &          100 &       99.5 &       97.9 &         99.3 \\
                  & switch15 &          100 &          100 &        100 &       98.6 &         99.7 \\
                  & switch15-limit &          100 &          100 &       99.5 &       98.4 &         99.5 \\
                  & OS/2 &         99.5 &         97.1 &       96.5 &       93.2 &         96.6 \\
                  & OS/2 &         99.5 &         97.1 &       96.7 &       92.9 &         96.6 \\
                  & OS/20 &          100 &          100 &        100 &       99.1 &         99.8 \\
                  & OS/20 &          100 &          100 &       99.5 &         99 &         99.6 \\
                  & switch25 &          100 &          100 &        100 &       99.3 &         99.8 \\
                  & switch25-limit &          100 &          100 &       99.5 &       99.2 &         99.7 \\
                  & OS/3 &          100 &         98.7 &       97.8 &       93.5 &         97.5 \\
                  & OS/3 &          100 &         98.7 &       97.8 &       93.1 &         97.4 \\
                  & OS/30 &          100 &          100 &        100 &       99.5 &         99.9 \\
                  & OS/30 &          100 &          100 &       99.5 &       99.5 &         99.7 \\
                  & switch35 &          100 &          100 &        100 &       99.5 &         99.9 \\
                  & switch35-limit &          100 &          100 &       99.5 &       99.5 &         99.8 \\
                  & OS/4 &          100 &         99.1 &       98.2 &       93.9 &         97.8 \\
                  & OS/4 &          100 &         99.1 &       98.8 &       93.8 &           98 \\
                  & OS/40 &          100 &          100 &        100 &       99.6 &         99.9 \\
                  & OS/40 &          100 &          100 &       99.5 &       99.6 &         99.8 \\
                  & switch5 &          100 &         99.5 &       98.9 &         95 &         98.4 \\
                  & switch5-limit &          100 &         99.5 &       99.3 &       95.5 &         98.6 \\
                  & switch6 &          100 &         99.7 &       99.3 &       95.8 &         98.7 \\
                  & switch6-limit &          100 &         99.7 &       99.3 &       95.9 &         98.7 \\
                  & switch7 &          100 &         99.8 &       99.6 &       96.6 &           99 \\
                  & switch7-limit &          100 &         99.8 &       99.5 &       96.7 &           99 \\
                  & switch8 &          100 &         99.9 &       99.7 &       97.1 &         99.2 \\
                  & switch8-limit &          100 &         99.9 &       99.6 &       97.2 &         99.2 \\
                  & switch9 &          100 &          100 &       99.8 &       97.5 &         99.3 \\
                  & switch9-limit &          100 &          100 &       99.6 &       97.4 &         99.2 \\
                  & WPP &         99.9 &         99.9 &       99.3 &       94.8 &         98.5 \\
                  & All &         99.7 &         99.2 &       98.9 &       96.7 &         98.6 \\
\bottomrule
\end{tabular}


==> figures/avail_size_mcmssp_limit_60.tex <==

\begin{tabular}{lllllll}
\toprule
                  & Avail. Agents & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{5} &          All \\
                  & Avail. Tasks & \multicolumn{2}{l}{20} & \multicolumn{3}{l}{20} \\
                  & agentavail & \multicolumn{2}{l}{100} & \multicolumn{3}{l}{100} \\
                  & taskavail &           50 &           75 &         50 & \multicolumn{2}{l}{75} \\
{} &  &              &              &            &            &              \\
\midrule
Rotational Diversity & FOA &  29.0 (45.4) &  28.0 (55.5) &  5.0 (7.7) &  5.0 (9.5) &  16.0 (29.5) \\
                  & PC &  30.0 (44.1) &  41.0 (49.8) &  6.0 (7.7) &  5.0 (9.1) &  20.0 (27.7) \\
                  & FOP &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  0.0 (8.6) &  14.0 (26.7) \\
                  & OS/1 &  32.0 (44.9) &  29.0 (55.5) &  4.0 (7.5) &  5.0 (9.4) &  17.0 (29.3) \\
                  & OS/10 &  27.0 (43.7) &  28.0 (47.8) &  2.0 (6.7) &  3.0 (8.8) &  15.0 (26.8) \\
                  & switch15-limit &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  2.0 (8.5) &  14.0 (26.7) \\
                  & OS/2 &  28.0 (44.0) &  36.0 (51.9) &  4.0 (7.2) &  5.0 (9.5) &  18.0 (28.2) \\
                  & OS/20 &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  1.0 (8.6) &  14.0 (26.7) \\
                  & switch25-limit &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  1.0 (8.6) &  14.0 (26.7) \\
                  & OS/3 &  27.0 (43.7) &  35.0 (50.0) &  4.0 (7.1) &  5.0 (9.4) &  17.0 (27.6) \\
                  & OS/30 &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  1.0 (8.6) &  14.0 (26.7) \\
                  & switch35-limit &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  0.0 (8.6) &  14.0 (26.7) \\
                  & OS/4 &  27.0 (43.7) &  31.0 (49.0) &  4.0 (7.0) &  5.0 (9.3) &  16.0 (27.2) \\
                  & OS/40 &  27.0 (43.7) &  27.0 (47.8) &  2.0 (6.7) &  0.0 (8.7) &  14.0 (26.7) \\
                  & switch5-limit &  27.0 (43.7) &  31.0 (48.4) &  4.0 (7.0) &  4.0 (8.8) &  16.0 (27.0) \\
                  & switch6-limit &  27.0 (43.7) &  29.0 (48.4) &  3.0 (6.9) &  4.0 (8.9) &  15.0 (27.0) \\
                  & switch7-limit &  27.0 (43.7) &  29.0 (48.2) &  3.0 (6.8) &  3.0 (8.7) &  15.0 (26.8) \\
                  & switch8-limit &  27.0 (43.7) &  28.0 (48.0) &  3.0 (6.9) &  3.0 (8.8) &  15.0 (26.8) \\
                  & switch9-limit &  27.0 (43.7) &  28.0 (48.0) &  3.0 (6.9) &  3.0 (8.8) &  15.0 (26.8) \\
                  & WPP &  30.0 (43.7) &  38.0 (48.4) &  5.0 (7.6) &  6.0 (9.1) &  19.0 (27.2) \\
                  & All &  27.0 (43.9) &  30.0 (49.2) &  3.0 (7.0) &  3.0 (8.9) &  15.0 (27.2) \\
Profit (\% of FOP) & FOA &         96.4 &           95 &         95 &       92.6 &         94.8 \\
                  & PC &         99.9 &         99.9 &       97.3 &       94.5 &         97.9 \\
                  & FOP &          100 &          100 &       99.5 &       99.8 &         99.8 \\
                  & OS/1 &         97.8 &         95.2 &       95.3 &       92.7 &         95.2 \\
                  & OS/10 &          100 &          100 &       99.5 &       97.9 &         99.3 \\
                  & switch15-limit &          100 &          100 &       99.5 &       98.4 &         99.5 \\
                  & OS/2 &         99.5 &         97.1 &       96.7 &       92.9 &         96.6 \\
                  & OS/20 &          100 &          100 &       99.5 &         99 &         99.6 \\
                  & switch25-limit &          100 &          100 &       99.5 &       99.2 &         99.7 \\
                  & OS/3 &          100 &         98.7 &       97.8 &       93.1 &         97.4 \\
                  & OS/30 &          100 &          100 &       99.5 &       99.5 &         99.7 \\
                  & switch35-limit &          100 &          100 &       99.5 &       99.5 &         99.8 \\
                  & OS/4 &          100 &         99.1 &       98.8 &       93.8 &           98 \\
                  & OS/40 &          100 &          100 &       99.5 &       99.6 &         99.8 \\
                  & switch5-limit &          100 &         99.5 &       99.3 &       95.5 &         98.6 \\
                  & switch6-limit &          100 &         99.7 &       99.3 &       95.9 &         98.7 \\
                  & switch7-limit &          100 &         99.8 &       99.5 &       96.7 &           99 \\
                  & switch8-limit &          100 &         99.9 &       99.6 &       97.2 &         99.2 \\
                  & switch9-limit &          100 &          100 &       99.6 &       97.4 &         99.2 \\
                  & WPP &         99.9 &         99.9 &         96 &       92.9 &         97.2 \\
                  & All &         99.7 &         99.2 &       98.5 &       96.4 &         98.4 \\
\bottomrule
\end{tabular}

